Meta-Reinforcement Learning Robust to Distributional Shift via Model Identification and Experience Relabeling

Reinforcement learning algorithms can acquire policies for complex tasks autonomously. However, the number of samples required to learn a diverse set of skills can be prohibitively large. While meta-reinforcement learning methods have enabled agents to leverage prior experience to adapt quickly to new tasks, their performance depends crucially on how close the new task is to the previously experienced tasks. Current approaches are either not able to extrapolate well, or can do so at the expense of requiring extremely large amounts of data for on-policy meta-training. In this work, we present model identification and experience relabeling (MIER), a meta-reinforcement learning algorithm that is both efficient and extrapolates well when faced with out-of-distribution tasks at test time. Our method is based on a simple insight: we recognize that dynamics models can be adapted efficiently and consistently with off-policy data, more easily than policies and value functions. These dynamics models can then be used to continue training policies and value functions for out-of-distribution tasks without using meta-reinforcement learning at all, by generating synthetic experience for the new task.

==> MIER - Arxiv/sections/conclusion.tex <==
\section{Conclusion}
In this paper, we introduce a consistent and sample efficient meta-RL algorithm by reformulating the meta-RL problem as \textbf{model identification}, and then described a method for adaptation to out-of-distribution tasks based on \textbf{experience relabeling}. Our algorithm can adapt to new tasks by determining the parameters of the model, which predicts the reward and future transitions, and can adapt \emph{consistently} to out-of-distribution tasks by adapting the model first, relabeling all data from the meta-training tasks with this model, and then finetuning on that data using a standard off-policy RL method. While \textbf{model identification} identification and \textbf{experience relabeling} can be used independently, with the former providing for a simple meta-RL framework, and the latter providing for adaptation to out-of-distribution tasks, we show that combining these components leads to good results across a range of challenging meta-RL problems that require extrapolating to out-of-distribution tasks at meta-test time.


==> MIER - Arxiv/sections/experiments.tex <==

\section{Experimental Evaluation} \label{sec:experiments}

We aim to answer the following questions in our experiments: \textbf{(1)} Can MIER meta-train efficiently on standard meta-RL benchmarks, with meta-training sample efficiency that is competitive with state-of-the-art methods? \textbf{(2)} How does MIER compare to prior meta-learning approaches for extrapolation to meta-test tasks with out-of-distribution (a) reward functions and (b) dynamics? \textbf{(3)} How important is experience relabeling in leveraging the model to train effective policies for out-of-distribution tasks?

To answer these questions, we first compare the meta-training sample efficiency of MIER to existing methods on several standard meta-RL benchmarks. We then test MIER on a set of out-of-distribution meta-test tasks to analyze extrapolation performance. We also compare against a version of our method without experience relabeling, in order to study the importance of this component for adaptation. All experiments are run with OpenAI gym~\citep{openaigym} and use the mujoco simulator~\citep{todorov2012mujoco}. We have released code to run our experiments at \url{https://github.com/russellmendonca/mier_public.git/}, and additional implementation and experiment details including hyperparameters are included in Appendix A.

\subsection{Meta-Training Sample Efficiency on Meta-RL Benchmarks}


We first evaluate MIER on standard meta-RL benchmarks, which were used in prior work~\citep{finn2017model,rakelly2019efficient,Fakoor2020Meta-Q-Learning}. Results are shown in Figure~\ref{fig:std_benchmark}.
We compare to PEARL~\citep{rakelly2019efficient}, which uses an off-policy encoder-based method, but without consistent adaptation, meta Q-learning (MQL)~\citep{Fakoor2020Meta-Q-Learning}, which also uses an encoder, MAML~\citep{finn2017model} and PRoMP~\citep{rothfuss2018promp}, which use MAML-based adaptation with on-policy policy gradients, and RL2~\citep{duan2016rl}, which uses an on-policy algorithm with an encoder.
We plot the meta-test performance after adaptation (on \textbf{in-distribution} tasks) against the number of meta-training samples, averaged across 3 random seeds. On these standard tasks, we run a variant of our full method which we call MIER-wR (MIER without \textbf{experience relabeling}), which achieves performance that is comparable to or better than the best prior methods, indicating that our \textbf{model identification} method provides a viable meta-learning strategy that compares favorably to state-of-the-art methods. However, the primary focus of our paper is on adaptation to \emph{out-of-distribution} tasks, which we analyze next.


\begin{figure}[t!]%
    \centering
   
    \includegraphics[width=0.245\linewidth]{sections/media/meta-training-benchmarks/cheetah-dir.png}
    \includegraphics[width=0.245\linewidth]{sections/media/meta-training-benchmarks/ant-dir.png}
    \includegraphics[width=0.245\linewidth]{sections/media/meta-training-benchmarks/humanoid-dir.png} 
    \includegraphics[width=0.235\linewidth]{sections/media/meta-training-benchmarks/walker-rand-params.png}
     \includegraphics[width=0.7\linewidth]{sections/media/legends/benchmarks_legend.png}
    
    \caption{\footnotesize Performance on standard meta-RL benchmarks. Return is evaluated over the course of the \emph{meta-training} process on meta-test tasks that are \textbf{in-distribution}. 
    }%
    \label{fig:std_benchmark}
\end{figure}

\subsection{Adaptation to Out-of-Distribution Tasks}\label{subsec:ood}

Next, we evaluate how well MIER can adapt to out-of-distribution, both on tasks with varying reward functions and tasks with varying dynamics.
We compare the performance of our full method (MIER), and MIER without experience relabeling (MIER-wR), to prior meta-learning methods for adaptation to out-of-distribution tasks. All algorithms are meta-trained with the same number of samples (2.5M for Ant Negated Joints, and 1.5M for all other domains) before evaluation. For performance of algorithms as a function of data used for meta-training, see Figure 6 in Appendix B.


\paragraph{Extrapolation over reward functions:} To evaluate extrapolation to out-of-distribution rewards, we first test on the half cheetah velocity extrapolation environments introduced by \citet{Fakoor2020Meta-Q-Learning}.\footnote{Since we do not have access to the code used by \citet{Fakoor2020Meta-Q-Learning}, quantitative results for the easier cheetah tasks are taken from their paper, but we cannot evaluate MQL on other more challenging tasks.} Half-Cheetah-Vel-Medium has training tasks where the cheetah is required to run at target speeds ranging from 0 to 2.5 m/s, while Half-Cheetah-Hard has training tasks where the target speeds are sampled from 0 to 1.5 m/s, as depicted in Figure~\ref{fig:cheetah_vel_task}. In both settings, the test set has target speeds sampled from 2.5 to 3 m/s.
In Figure~\ref{fig:ood}, we see that our method matches MQL on the easier Half-Cheetah-Vel-Medium environment, and outperforms all prior methods including MQL on the Half-Cheetah-Vel-Hard setting, where extrapolation is more difficult. Furthermore we see that experience relabeling improves performance for our method for both settings.

We also evaluate reward function extrapolation for an Ant that needs to move in different directions, with the training set comprising directions sampled from 3 quarters of a circle, and the test set containing tasks from the last quadrant, as shown in Figure~\ref{fig:ant_dir_task}. We see in Figure~\ref{fig:ood} that our method outperforms prior algorithms by a large margin in this setting.
We provide a more fine-grained analysis of adaptation performance on different tasks in the test set in Figure~\ref{fig:ood_sensitivity}. We see that while the performance of all methods degrades as validation tasks get farther away from the training distribution, MIER and MIER-wR perform consistently better than MAML and PEARL. 


\begin{figure}[t!]%
    \centering
   
    \subfigure[\scriptsize Cheetah Velocity]{\label{fig:cheetah_vel_task}\includegraphics[width=0.245\linewidth]{sections/media/task_figures/cheetah-vel.png}}
    \subfigure[\scriptsize Ant Direction]{\label{fig:ant_dir_task}\includegraphics[width=0.245\linewidth]{sections/media/task_figures/ant-dir.png}}
    \subfigure[\scriptsize Cheetah Negated Joints]{\label{fig:cheetah_neg_task}\includegraphics[width=0.245\linewidth]{sections/media/task_figures/cheetah-negated.png}}
    \subfigure[\scriptsize Ant Negated Joints]{\label{fig:ant_neg_task}\includegraphics[width=0.245\linewidth]{sections/media/task_figures/ant-negated.png}}
    
    \caption{\footnotesize Illustration of out-of-distribution adaptation tasks: (a) Cheetah-Velocity Medium (target velocity training set in blue, test set in red) and Cheetah-Velocity Hard (target velocity training set in green, test set in red), (b) Ant Direction (target direction training tasks in green, test tasks in red), (c) Cheetah Negated Joints and (d) Ant Negated Joints. Training and test sets are indicated in the figure for (a) and (b). In the negated joint environments, the control is negated to a set of randomly selected joints, and the movement direction when control is applied is depicted for both negated and normal joints.
    }%
    \label{fig:tasks}
\end{figure}

\begin{figure}[t!]%
    \centering
   
    \includegraphics[width=0.32\linewidth]{sections/media/ood-bar-plots/cheetah-vel-medium.png}
    \includegraphics[width=0.32\linewidth]{sections/media/ood-bar-plots/cheetah-vel-hard.png}
    \includegraphics[width=0.32\linewidth]{sections/media/ood-bar-plots/ant-dir.png}
    \includegraphics[width=0.32\linewidth]{sections/media/ood-bar-plots/cheetah-negated-joints.png} 
    \includegraphics[width=0.32\linewidth]{sections/media/ood-bar-plots/ant-negated-joints.png}
    \includegraphics[width=0.9\linewidth]{sections/media/legends/ood_bar_plot_legend.png}
    \caption{\footnotesize Performance on out-of-distribution tasks. All algorithms are meta-trained with the same amount of data, and then evaluated on out-of-distribution tasks. Cheetah-Velocity and Ant-Direction environments have varying reward functions, while Cheetah-Negated-Joints and Ant-Negated-Joints have different dynamics.
    }%
    \label{fig:ood}
\end{figure}

\begin{figure}[t!]%
    \centering
   
    \includegraphics[width=0.3\linewidth]{sections/media/ood/cheetah-vel-sensitivity.png}
    \includegraphics[width=0.3\linewidth]{sections/media/ood/ant-dir-sensitivity.png}
     \includegraphics[width=0.6\linewidth]{sections/media/legends/ood_sensitivity_legend.png}
   
    \caption{\footnotesize Performance evaluated on validation tasks of varying difficulty. For Cheetah Velocity, the training distribution consists of target speeds from 0 to 1.5 m/s, and so tasks become harder left to right along the x axis. Ant Direction consists of training tasks ranging from 0 to 1.5 $\pi$ radians, so the hardest tasks are in the middle.  
    }%
    \label{fig:ood_sensitivity}
\end{figure}


\paragraph{Extrapolation over dynamics:} To study adaptation to out-of-distribution dynamics, we constructed variants of the HalfCheetah and Ant environments where we randomly negate the control of randomly selected groups of joints as shown in Figures ~\ref{fig:cheetah_neg_task} and ~\ref{fig:ant_neg_task}. During meta-training, we never negate the last joint, such that we can construct out-of-distribution tasks by negating this last joint, together with a randomly chosen subset of the others. For the HalfCheetah, we negate 3 joints at a time from among the first 5 during meta-training, and always negate the 6th joint (together with a random subset of 2 of the other 5) for testing, such that there are 10 meta-training tasks and 10 out-of-distribution evaluation tasks. For the Ant, we negate 4 joints from among the first 7 during meta-training, and always negate the 8th (together with a random subset of 3 of the other 7) for evaluation, resulting in 35 meta-training tasks and 35 evaluation tasks, out of which we randomly select 15.

In addition to PEARL and MAML, we compare against GrBAL~\citep{nagabandi2018learning}, a model based meta-RL method. We note that we could not evaluate GrBAL on the reward extrapolation tasks, since it requires the analytic reward function to be known during planning, but we can compare to this method under varying dynamics.
From Figure~\ref{fig:ood}, we see that performance on Cheetah-Negated-Joints with just context adaptation (MIER-wR) is substantially better than PEARL and MAML and GrBAL, and there is further improvement by using the model for relabeling (MIER). On the more challenging Ant-Negated-Joints environment, MIER-wR shows similar performance to PEARL, and leveraging the model for relabeling again leads to better performance for MIER.




==> MIER - Arxiv/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Recent advances in reinforcement learning (RL) have enabled agents to autonomously acquire policies for complex tasks, particularly when combined with high-capacity representations such as neural networks ~\citep{lillicrap2015continuous, schulman2015trust, mnih2015human, levine2016end}. However, the number of samples required to learn these tasks is often very large. Meta-reinforcement learning (meta-RL) algorithms can alleviate this problem by leveraging experience from previously seen related tasks~\citep{duan2016rl,Wang2016LearningTR,finn2017model}, but the performance of these methods on new tasks depends crucially on how close these tasks are to the meta-training task distribution. Meta-trained agents can adapt quickly to tasks that are similar to those seen during meta-training, but lose much of their benefit when adapting to tasks that are too far away from the meta-training set. This places a significant burden on the user to carefully construct meta-training task distributions that sufficiently cover the kinds of tasks that may be encountered at test time.


Many meta-RL methods either utilize a variant of model-agnostic meta-learning (MAML) and adapt to new tasks with gradient descent~\citep{finn2017model,rothfuss2018promp,nagabandi2018learning}, or use an encoder-based formulation that adapt by encoding experience with recurrent models~\citep{duan2016rl, Wang2016LearningTR}, attention mechanisms~\citep{mishra2017simple} or variational inference~\citep{rakelly2019efficient}. The latter class of methods generally struggle when adapting to out-of-distribution tasks, because the adaptation procedure is entirely learned and carries no performance guarantees with out-of-distribution inputs (as with any learned model). Methods that utilize gradient-based adaptation have the potential of handling out-of-distribution tasks more effectively, since gradient descent corresponds to a well-defined and consistent learning process that has a guarantee of improvement regardless of the task~\citep{finn2018metalearning}. However, in the RL setting, these methods~\citep{finn2017model,rothfuss2018promp} utilize on-policy policy gradient methods for meta-training, which require a very large number of samples during meta-training~\citep{rakelly2019efficient}.


In this paper, we aim to develop a meta-RL algorithm that can both adapt effectively to out-of-distribution tasks and be meta-trained efficiently via off-policy value-based algorithms. One straightforward idea might be to directly develop a value-based off-policy meta-RL method that uses gradient-based meta-learning. However, this is very difficult, since the fixed point iteration used in value-based RL algorithms does not correspond to gradient descent, and to our knowledge no prior method has successfully adapted MAML to the off-policy value-based setting. We further discuss this difficulty in Appendix ~\ref{app:maml_q_learning}. Instead, we propose to leverage a simple insight: \emph{dynamics and reward models} can be adapted consistently, using gradient based update rules with off-policy data, even if policies and value functions cannot. These models can then be used to train policies for out-of-distribution tasks without using meta-RL at all, by generating synthetic experience for the new tasks.


Based on this observation, we propose \textbf{model identification and experience relabeling} (MIER), a meta-RL algorithm that makes use of two independent novel concepts: \textbf{model identification} and \textbf{experience relabeling}. Model identification refers to the process of identifying a particular task from a distribution of tasks, which requires determining its transition dynamics and reward function. We use a gradient-based \emph{supervised} meta-learning method to learn a dynamics and reward model and a (latent) \emph{model context variable} such that the model quickly adapts to new tasks after a few steps of gradient descent on the context variable.
The context variable must contain sufficient information about the task to accurately predict dynamics and rewards. The policy can then be conditioned on this context ~\citep{universalValueFunc, Kaelbling1993LearningTA} and therefore does \emph{not} need to be meta-trained or adapted. Hence it can be learned with any standard RL algorithm, avoiding the complexity of meta-reinforcement learning. We illustrate the model identification process in the left part of Figure \ref{fig:introFig}.


\begin{figure}[t!]%
    \centering
   
    \includegraphics[width=0.45\linewidth]{sections/media/intro_figures/model_id.png}
    \includegraphics[width=0.45\linewidth]{sections/media/intro_figures/relabel_exp.png}
     
    \caption{\footnotesize Overview of our approach. The model context variable ($\phi$) is adapted using gradient descent, and the adapted context variable ($\phi_{\task}$) is fed to the policy alongside state so the policy can be trained with standard RL (Model Identification). The adapted model is used to relabel the data from other tasks by predicting next state and reward, generating synthetic experience to continue improving the policy (Experience Relabeling).
    }%
    \label{fig:introFig}
\end{figure}


When adapting to out-of-distribution tasks at meta-test time, the adapted context variable may itself be out of distribution, and the context-conditioned policy might perform poorly. However, since MIER adapts the model with gradient descent, we can continue to improve the model using more gradient steps. To continue improving the policy, we leverage all data collected from other tasks during meta-training, by using the learned model to \emph{relabel} the next state and reward on every previously seen transition, obtaining synthetic data to continue training the policy. We call this process, shown in the right part of Figure \ref{fig:introFig}, \textbf{experience relabeling}. This enables MIER to adapt to tasks outside of the meta-training distribution, outperforming prior meta-reinforcement learning methods in this setting.


==> MIER - Arxiv/sections/method.tex <==
\section{Meta Training with Model Identification}

As discussed in Section~\ref{sec:intro}, MIER is built on top of two concepts, which we call \textbf{model identification} and \textbf{experience relabeling}. We first discuss how we can reformulate the meta-RL problem into a model identification problem, where we train a fast-adapting model to rapidly identify the transition dynamics and reward function for a new task. We parameterize the model with a latent context variable, which is meta-trained to encapsulate all of the task-specific information acquired during adaptation. We then train a universal policy that, conditioned on this context variable, can solve all of the meta-training tasks. Training this policy is a standard RL problem instead of a meta-RL problem, so any off-the-shelf off-policy algorithms can be used. The resulting method can immediately be used to adapt to new in-distribution tasks, simply by adapting the model's context via gradient descent, and conditioning the universal policy on this context. We illustrate the model identification part of our algorithm in the left part of Figure \ref{fig:introFig} and provide pseudo-code for our meta-training procedure in Algorithm \ref{alg:meta_train}.


In a meta-RL problem, where tasks are sampled from a distribution of MDPs, the only varying factors are the dynamics $p$ and the reward function $r$. Therefore, a sufficient condition for identifying the task is to learn the transition dynamics and the reward function, and this is exactly what model-based RL methods do. Hence, we can naturally formulate the meta-task identification problem as a model-based RL problem and solve it with supervised meta-learning methods.


Specifically, we choose the MAML method for its simplicity and consistency. Unlike the standard supervised MAML formulation, we condition our model on a latent context vector, and we only change the context vector when adapting to new tasks. Since all task-specific information is thus encapsulated in the context vector, conditioning the policy on this context should provide it with sufficient information to solve the task. This architecture is illustrated in the left part of Figure~\ref{fig:introFig}. We denote the model as $\model(\nextstate, \reward | \state, \action; \theta, \phi)$, where $\theta$ is the neural network parameters and $\phi$ is the latent context vector that is passed in as input to the network.

One step of gradient adaptation can be written as follows:

\begin{equation*}
\label{context update}
\phi_{\task} = \mamladaptation \left(\theta, \phi, \data^{ \left(\task \right)}_{adapt} \right)
= \phi - \alpha \nabla_{\phi} \mathbb{E}_{ \left(\state, \action, \nextstate, \reward \right)  \sim \data^{ \left(\task \right)}_{adapt}} [-\log \model \left(\nextstate, \reward | \state, \action; \theta, \phi \right) ].
\end{equation*}
We use the log likelihood as our objective for the probabilistic model. We then evaluate the model using the adapted context vector $\phi_\task$, and minimize its loss on the evaluation dataset to learn the model. Specifically, we minimize the model meta-loss function $\modelloss(\theta, \phi, \data^{(\task)}_{adapt}, \data^{(\task)}_{eval})$ to obtain the optimal parameter $\theta$ and context vector initialization $\phi$:
\begin{equation*}
\label{meta train objective}
% \begin{align*}
    \arg\min_{\theta, \phi} \modelloss \left(\theta, \phi, \data^{\left(\task\right)}_{adapt}, \data^{\left(\task\right)}_{eval}\right)
    = \arg\min_{\theta, \phi} \mathbb{E}_{\left(\state, \action, \nextstate, \reward\right)  \sim \mathcal{D}^{\left(\task\right)}_{eval}} [-\log \model\left(\nextstate, \reward | \state, \action; \theta, \phi_{\task}\right)]
% \end{align*}
\end{equation*}
The main difference between our method and previously proposed meta-RL methods that also use context variables~\citep{rakelly2019efficient, duan2016rl} is that we use gradient descent to adapt the context. Adaptation will be much faster for tasks that are in-distribution, since the meta-training process explicitly optimizes for this objective, but the model will still adapt to out-of-distribution tasks given enough samples and gradient steps, since the adaptation process corresponds to a well-defined and convergent learning process. However, for out-of-distribution tasks, the adapted context could be out-of-distribution for the policy. We address this problem in Section~\ref{sec:relab}.


\begin{wrapfigure}{r}{0.5\textwidth}

\vspace{-0.3in}

\noindent
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
  \footnotesize
  \begin{flushleft}
        \textbf{Input:} task distribution $\taskdistribution(\task)$, training steps $N$, learning rate $\alpha$ \\
        \textbf{Output:} policy parameter $\psi$, model parameter $\theta$, model context $\phi$
  \end{flushleft}
  Randomly initialize $\psi$, $\theta$, $\phi$ \; \\
  Initialize multitask replay buffer $\mathcal{R}(\task) \leftarrow \emptyset$ \; \\
  \While{$\theta$, $\phi$, $\psi$ not converged}{
    Sample task $\task \sim \taskdistribution(\task)$ \; \\
    Collect $\data^{(\task)}_{adapt}$ using $\policy_{\psi}$ and $\phi$ \; \\
    Compute $\phi_{\task} = \mamladaptation(\theta, \phi, \data^{(\task)}_{adapt})$ \; \\
    Collect $\data^{(\task)}_{eval}$ using $\policy$ and $\phi_{\task}$ \; \\
    $\mathcal{R}(\task) \leftarrow \mathcal{R}(\task) \cup \data^{(\task)}_{adapt} \cup \data^{(\task)}_{eval}$ \; \\
    \For{$i$ = $1$ to $N$}{
        Sample task $\task \sim \mathcal{R}$ \; \\
        Sample $\data^{(\task)}_{adapt}, \data^{(\task)}_{eval} \sim  \mathcal{R}(\task)$ \; \\
        Update $\theta \leftarrow \theta - \alpha \nabla_{\theta} \modelloss(\theta, \phi, \data^{(\task)}_{adapt}, \data^{(\task)}_{eval}) $ \; \\
        % Compute $\phi_{\task} = \mamladaptation(\theta, \phi, \data^{(\task)}_{adapt})$ \; \\
        Update $\psi \leftarrow \psi - \alpha \nabla_{\psi} \policyloss(\psi, \data^{(\task)}_{eval}, \phi_{\task})$ \; \\
    }
  }
  \caption{Model Identification Meta-Training}
  \label{alg:meta_train}
\end{algorithm}
\end{minipage}
\noindent
\vspace{-0.05in}
\end{wrapfigure}


Given the latent context variable from the adapted model $\phi_{\task}$, the meta-RL problem can be effectively reduced to a standard RL problem, as the task specific information has been encoded in the context variable.
We can therefore apply any standard model-free RL algorithm to obtain a policy, as long as we condition the policy on the latent context variable.

In our implementation, we utilize the soft actor-critic (SAC) algorithm~\citep{haarnoja2018soft}, though any efficient model-free RL method could be used. We briefly introduce the policy optimization process for a general actor-critic method. Let us parameterize our policy $\policy_{\psi}$ by a parameter vector $\psi$. Actor-critic methods maintain an estimate of the Q values for the current policy,
$Q^{\policy_{\psi}}(\state, \action, \phi_{\task}) =
\mathbb{E}_{\state_t, \action_t \sim \policy_{\psi}}[\sum_t \discount^t \rewardfunc(\state_t, \action_t) | \state_0 = \state, \action_0 = \action, \task]
$,
via Bellman backups, and improve the policy by maximizing the expected Q values under the policy, averaged over the dataset $\data$. The policy loss can be written as: 
\begin{equation*}
\policyloss(\psi, \data, \phi_{\task} ) = -\mathbb{E}_{\state \sim \data, \action \sim \policy}[Q^{\policy_{\psi}}(\state, \action, \phi_{\task})]
\end{equation*}
Note that we condition our value function $Q^{\policy_{\psi}}(\state, \action, \phi_\task)$ and policy $\policy_{\psi}(\action | \state, \phi_\task)$ on the adapted task specific context vector $\phi_{\task}$, so that the policy and value functions are aware of which task is being performed~\citep{universalValueFunc, Kaelbling1993LearningTA}. Aside from incorporating the context $\phi_\task$, the actual RL algorithm is unchanged, and the main modification is the concurrent meta-training of the model to produce $\phi_\task$.


\section{Improving Out-of-Distribution Performance by Experience Relabeling} \label{sec:relab}


At meta-test time, when our method must adapt to a new unseen task $\task$, it will first sample a small batch of data and obtain the latent context $\phi_{\task}$ by running the gradient descent adaptation process on the context variable, using the model identification process introduced in the previous section. While our model identification method is already a complete meta-RL algorithm, it has no guarantees of consistency. That is, it might not be able to adapt to out-of-distribution tasks, even with large amounts of data: although the gradient descent adaptation process for the model is consistent and will continue to improve, the context variable $\phi_{\task}$ produced by this adaptation may still be out-of-distribution for the policy when adapting to an out-of-distribution task. However, with an improved model, we can continue to train the policy with standard off-policy RL, by generating synthetic data using the model. In practice we adapt the model for as many gradient steps as necessary, and then use this model to generate synthetic transitions using states from all previously seen meta-training tasks, with new successor states and rewards. We call this process experience relabeling. Since the model is adapted via gradient descent, it is guaranteed to eventually converge to a local optimum for any new task, even a task that is outside the meta-training distribution. We illustrate the experience relabeling process in the right part of Figure \ref{fig:introFig}, and provide pseudo-code in Algorithm \ref{alg:adapt}.

\begin{wrapfigure}{r}{0.52\textwidth}

\vspace{-0.33in}

\begin{minipage}{0.52\textwidth}
\begin{algorithm}[H]
\label{alg:metaopt}
    \footnotesize

    \begin{flushleft}
        \textbf{Input:} test task $\hat{\task}$, multitask replay buffer $\mathcal{R}(\task)$, Adaptation steps for context $N_{fast}$, Training steps for policy $N_p$, Training steps for model $N_m$ \\
        \textbf{Output:} policy parameter $\psi$
    \end{flushleft}
  
  Collect $\data^{(\hat{\task})}_{adapt}$ from $\hat{\task}$ using $\policy_{\psi}$ and $\phi$ \; \\
  \For{$i$ = $1$ to $N_{fast}$}{
        Update $\phi_{\task}$ according to Eq. ~\ref{context update}
    }
  \While{$\psi$ not converged}{
 
    \For{$i$ = $1$ to $N_p$}{
        Sample $\task \sim \mathcal{R}$ and 
        $\data^{(\task)} \sim  \mathcal{R}(\task)$ \; \\
        $\hat\data^{(\hat{\task})} \leftarrow \relabel(\data^{(\task)}, \theta, \phi_{\hat{\task}})$ \; \\
        Train policy $\psi \leftarrow \psi - \alpha \nabla_{\psi} \policyloss(\psi, \hat\data^{(\hat{\task})}, \phi_{\task}  )$ \; \\
    }
  
  }
  \caption{Experience Relabeling Adaptation}
  \label{alg:adapt}
\end{algorithm}
\end{minipage}
\vspace{-0.2in}
\end{wrapfigure}



When using data generated from a learned model to train a policy, the model's predicted trajectory often diverges from the real dynamics after a large number of time steps, due to accumulated error~\citep{janner2019trust}. We can mitigate this issue in the meta-RL case by leveraging all of the data from other tasks that was available during meta-training. Although new task is previously unseen, the other training tasks share the same state space and action space, and so we can leverage the large set of diverse transitions collected from these tasks. Using the adapted model and policy, we can \emph{relabel} these transitions, denoted $(\state, \action, \nextstate, \reward)$, by sampling new actions with our adapted policy, and by sampling next states and rewards from the adapted model.
The relabeling process can be written as: 
\begin{equation*}
\relabel(\data, \theta, \phi_{\task}) = \{(\state, \action, \nextstate, \reward) | \state \in \data; \action \sim \policy(\action | \state, \phi_{\task}), (\nextstate, \reward) \sim \model(\nextstate, \reward | \state, \action; \theta, \phi_{\task})\}.
\end{equation*}

We use these relabeled transitions to continue training the policy. The whole adaptation process is summarized in Algorithm \ref{alg:adapt}. 
Since the learned model is only used to predict one time step into the future, our approach does not suffer from compounding model errors. 
The MQL algorithm \citep{Fakoor2020Meta-Q-Learning} also reuses data from other training tasks, but requires re-weighting them with an estimated importance ratio instead of relabeling them with an adapted model. We will show empirically that our approach performs better on out-of-distribution tasks, and we also note that such reweighting could be infeasible in some environments, which we discuss in Appendix C. We also note that our experience relabeling method is a general tool for adapting to out-of-distribution tasks, and could be used independently of our model identification algorithm. For example, we could apply a standard, non-context-based dynamics and reward model to generate synthetic experience to finetune a policy obtained from any source, including other meta-RL methods.


==> MIER - Arxiv/sections/preliminaries.tex <==
\section{Preliminaries}

Formally, the reinforcement learning problem is defined by a Markov decision process (MDP). We adopt the standard definition of an MDP, $\task = (\statespace, \actionspace, \transition, \initialstate, \rewardfunc, \discount)$, where $\statespace$ is the state space, $\actionspace$ is the action space, $\transition(\nextstate|\state,\action)$ is the unknown transition probability of reaching state $\nextstate$ at the next time step when an agent takes action $\action$ at state $\state$, $\initialstate(\state)$ is the initial state distribution, $\rewardfunc(\state, \action)$ is the reward function, and $\discount \in (0, 1)$ is the discount factor. An agent acts according to some policy $\policy(\action|\state)$ and the learning objective is to maximize the expected return, $\mathbb{E}_{\state_t, \action_t \sim \policy}[\sum_t \discount^t \rewardfunc(\state_t, \action_t)]$.

We further define the meta-reinforcement learning problem. Meta-training uses a distribution over MDPs, $\taskdistribution(\task)$, from which tasks are sampled. Given a specific task $\task$, the agent is allowed to collect a small amount of data $\mathcal{D}^{(\task)}_{adapt}$, and adapt the policy to obtain $\pi_{\task}$. The objective of meta-training is to maximize the expected return of the adapted policy $\mathbb{E}_{\task \sim \taskdistribution(\task), \state_t, \action_t \sim \pi_{\task}}[\sum_t \discount^t \rewardfunc(\state_t, \action_t)]$.

MIER also makes use of a learned dynamics and reward model, similar to model-based reinforcement learning. In model-based reinforcement learning, a model $\hat{p}(\nextstate, \reward|\state,\action)$
that predicts the reward and next state from current state and action is trained using supervised learning. The model may then be used to generate data to train a policy, using an objective similar to the RL objective above:
$\arg\max_{\pi} \mathbb{E}_{\state_t, \action_t \sim \policy, \hat{p}}[\sum_t \gamma^t \rewardfunc(\state_t, \action_t)]$.
Note that the expectation is now taken with respect to the policy and learned model, rather than the policy and the true MDP transition function $\transition(\nextstate|\state,\action)$.


In order to apply model-based RL methods in meta-RL, we need to solve a supervised meta-learning problem. We briefly introduce the setup of supervised meta-learning and the model agnostic meta-learning approach, which is an important foundation of our work. In supervised meta-learning, we also have a distribution of tasks $\taskdistribution(\task)$ similar to the meta-RL setup, except that the task $\task$ is now a pair of input and output random variables $(X_{\task}, Y_{\task})$. Given a small dataset $\mathcal{D}^{(\task)}_{adapt}$ sampled from a specific task $\task$, the objective is to build a model that performs well on the evaluation data $\mathcal{D}^{(\task)}_{eval}$ sampled from the same task. If we denote our model as $f(X; \theta)$, the adaptation process as $\adaptation(\theta, \mathcal{D}^{(\task)}_{adapt})$ and our loss function as $\mathcal{L}$, the objective can be written as:
\vspace{-0.4cm}

$$\min_{f, \adaptation} \mathbb{E}_{\task \sim \taskdistribution \left(\task \right)} \left[\mathcal{L} \left(f \left(X_\task; \adaptation \left(\theta, \mathcal{D}^{ \left(\task \right)}_{adapt} \right) \right), Y_\task \right) \right]$$

\vspace{-0.2cm}

Model agnostic meta-learning \citep{finn2017model} is an approach to solve the supervised meta-learning problem. Specifically, the model $f(X; \theta)$ is represented as a neural network, and the adaptation process is represented as few steps of gradient descent. For simplicity of notation, we only write out one step of gradient descent:

\vspace{-0.4cm}

$$\mamladaptation \left(\theta, \mathcal{D}^{ \left(\task \right)}_{adapt} \right) = \theta - \alpha \nabla_{\theta} \mathbb{E}_{X, Y \sim \mathcal{D}^{ \left(\task \right)}_{adapt}} \left[\mathcal{L} \left(f \left(X; \theta \right), Y \right) \right]
$$
\vspace{-0.4cm}

The training process of MAML can be summarized as optimizing the loss of the model after few steps of gradient descent on data from the new task. Note that because $\mamladaptation$ is the standard gradient descent operator, our model is guaranteed to improve under suitable smoothness conditions regardless of the task distribution $\taskdistribution(\task)$, though adaptation to in-distribution tasks is likely to be substantially more efficient.



==> MIER - Arxiv/sections/related_work.tex <==
\section{Related Work}


Meta-reinforcement learning algorithms extend the framework of meta-learning~\citep{schmidhuber1987evolutionary,thrun1998learning,naik1992meta, bengio1990learning} to the reinforcement learning setting. 
Model-free encoder-based methods, encode the transitions seen during adaptation into a latent context variable, and the policy is conditioned on this context to adapt it to the new task. The context encoding process is often done via a recurrent network \citep{duan2016rl, Wang2016LearningTR, Fakoor2020Meta-Q-Learning, stadie2018some}, an attention mechanism \citep{mishra2017simple}, or via amortized variational inference \citep{rakelly2019efficient, humplik2019meta}. 
While inference is efficient for handling in-distribution tasks (Fig. \ref{fig:std_benchmark}), it is not effective for adaptation to out-of-distribution tasks (Fig. \ref{fig:ood}).
On the other hand, MIER can handle out-of-distribution tasks through the use of a consistent gradient descent learner for the model, followed by a consistent (non-meta-trained) off-policy reinforcement learning method.

Model-free gradient-based meta-RL methods \citep{finn2017model, rothfuss2018promp, zintgraf2018caml, rusu2018meta, liu2019taming, gupta2018meta, metacritic, houthooft2018evolved}, implement gradient descent as the adaptation process. However, they are based on on-policy RL algorithms, and thus require a large number of samples for training and adaptation (Fig. \ref{fig:std_benchmark}).  
There are also works that combine gradient-based and context-based methods \citep{lan2019meta}. However, such methods still suffer from the same sample efficiency problem as other gradient based methods, because of the use of on-policy policy gradients. Our method mitigates this problem by combining a gradient-based supervised meta-learning algorithm with a regular RL algorithm to achieve better sample efficiency at meta-training time. There has been some work that uses off-policy policy gradients for sample efficient meta-training ~\citep{gmps}, but this still requires quite a few trajectories for policy gradient based adaptation at test time.
MIER avoids this by reusing the experiences collected during training to enable fast adaptation with minimal amount of additional data.

Model based meta-RL methods meta-train a model rather than a policy \citep{nagabandi2018learning, saemundsson2018meta}. 
At test time, when the model is adapted to a particular task, standard planning techniques, such as model predictive control ~\cite{mppi, mpc}, are often applied to select actions. Unfortunately, purely model-based meta-RL methods typically attain lower overall returns than their model-free counter-parts, particularly for long-horizon tasks. Our method can attain comparatively higher final returns, since we only use one-step predictions from our model to provide synthetic data for a model-free RL method (Fig. \ref{fig:ood}). This resembles methods that combine model learning with model-free RL in single-tasks settings~\citep{sutton1991dyna, janner2019trust}.

